Unremarkable to Remarkable AI Agent: Exploring Boundaries of Agent Intervention for Adults With and Without Cognitive Impairment

As the population of older adults increases, there is a growing need for support for them to age in place. This is exacerbated by the growing number of individuals struggling with cognitive decline and shrinking number of youth who provide care for them. Artificially intelligent agents could provide cognitive support to older adults experiencing memory problems, and they could help informal caregivers with coordination tasks. To better understand this possible future, we conducted a speed dating with storyboards study to reveal invisible social boundaries that might keep older adults and their caregivers from accepting and using agents. We found that healthy older adults worry that accepting agents into their homes might increase their chances of developing dementia. At the same time, they want immediate access to agents that know them well if they should experience cognitive decline. Older adults in the early stages of cognitive decline expressed a desire for agents that can ease the burden they saw themselves becoming for their caregivers. They also speculated that an agent who really knew them well might be an effective advocate for their needs when they were less able to advocate for themselves. That is, the agent may need to transition from being unremarkable to remarkable. Based on these findings, we present design opportunities and considerations for agents and articulate directions of future research.

==> participants_table.tex <==
\begin{table}[H]
%[httt]
	\centering
    \small
	\begin{tabular}{p{0.3\textwidth}  p{0.17\textwidth}  p{0.17\textwidth}} 
 \textbf{Description} & \textbf{Healthy \newline Participants \newline (n=16)} & \textbf{Participants with \newline Memory Problems \& \newline Caretakers (n=18)} \\ 

    \toprule
 
 Type of study sessions & 
 16 individuals & 9 pairs \\
 
 \midrule
 
Female \newline Male & 
13 \newline 3 & 10 \newline 8\\ 

 \midrule
 
Age (Min) \newline Age (Max) \newline Age(Mean) & 
64 \newline 84 \newline 73.93 &
20 \newline 83 \newline 65.67\\ 

 \midrule
 
  Who do you live with? \newline Alone \newline With Spouse \newline With Spouse + Children \newline With Spouse + Friend \newline With Child(ren) \newline With Other Family \newline With Friend(s) \newline Did not share& 
 -- \newline 7 \newline 2 \newline 1 \newline 0 \newline 0 \newline 0 \newline 0 \newline 6 & 
 -- \newline 1 \newline 8 \newline 3 \newline 2 \newline 2 \newline 2 \newline 0 \newline 0 \\


 \midrule
 
 Need help with daily cognitive tasks? \newline Yes \newline No & 
 -- \newline 4 \newline 11 &
 -- \newline 9 \newline 9\\

 \midrule
 Experiencing memory problems \newline that are worsening over time?
 \newline Yes \newline No &
 -- \newline -- \newline 7 \newline 9 &
 -- \newline -- \newline 14 \newline 4 \\

  \midrule
 
 Support an older adult who needs \newline help with daily cognitive tasks? \newline Yes \newline No & 
 -- \newline -- \newline 2 \newline 14 &
 -- \newline -- \newline 11 \newline 7\\

   \midrule
 
 Support an older adult who is \newline experiencing memory problems? \newline Yes \newline No & 
 -- \newline -- \newline 3 \newline 13 &
 -- \newline -- \newline 11 \newline 7\\

    \midrule
 
 Diagnosed with memory loss (e.g., MCI)? \newline Yes \newline No \newline Prefer not to say & 
 -- \newline 0 \newline 16 \newline 0 &
 -- \newline 2 \newline 15 \newline 1\\

    \midrule
 
 Diagnosed with early dementia? \newline Yes \newline No & 
 -- \newline 0 \newline 16 &
 -- \newline 1 \newline 17 \\

 \bottomrule
 
 \end{tabular}
 \caption{Summary of participants' demographics: We interviewed 34 participants who belong to one of the two groups. The first group was 16 healthy, individual older adults and the second group was 9 pairs consisting of an older adult with memory problems and their caregiver. Some caregivers also had concerns about their own memory, but they were asked to focus on the person they support.}
 \label{tab:participants_table}
 \end{table}

==> participants_table_mci.tex <==
\begin{table}[H]
%[httt]
	\centering
    \small
	\begin{tabular}{p{0.3\textwidth}  p{0.17\textwidth}} 
 \textbf{Description} & \textbf{Participants with \newline Memory Problems} \\ 

    \toprule
 
 %Who do you live with? \newline Alone \newline Spouse \newline Spouse \& Children \newline Spouse \& Friend \newline Child(ren) \newline Other Family & 
 %-- \newline 1 \newline 8 \newline 3 \newline 2 \newline 2 \newline 2 \\

    \midrule

Do you have a smart phone? \newline Yes \newline No \newline Used To &
-- \newline 16 \newline 1 \newline 1 \\

 \bottomrule
 
 \end{tabular}
 \caption{Participants with memory problems' and their caregivers' demographics information.}
 \label{tab:participants_table_mci}
 \end{table}
